Toward Foraging for Understanding of StarCraft Agents: An Empirical Study

Assessing and understanding intelligent agents is a difficult task for users that lack an AI background. A relatively new area, called "Explainable AI," is emerging to help address this problem, but little is known about how users would forage through information an explanation system might offer. To inform the development of Explainable AI systems, we conducted a formative study, using the lens of Information Foraging Theory, into how experienced users foraged in the domain of StarCraft to assess an agent. Our results showed that participants faced difficult foraging problems. These foraging problems caused participants to entirely miss events that were important to them, reluctantly choose to ignore actions they did not want to ignore, and bear high cognitive, navigation, and information costs to access the information they needed.

==> leftovers.tex <==
\section{LEFTOVERS, DO NOT BE RENDERING THIS SECTION IN FINAL COPY}

\boldify{So, what does that buy us? First, it lets us see the forest for the trees: 1. It unifies RQ1 w RQ2 by showing the sometimes large navigational foraging effort for the prey in RQ1, with the sometimes large cognitive foraging effort in RQ2.  2. It unifies RQ2 and RQ3 by considering that both address WHY the participant is doing the WRONG thing, one is based on losing PREY in the shuffle, while the other is based on something screwing up value/cost estimation. }

In the RTS domain, going individual paths, like in the right half of \ref{fig:paths}, generally had a small cost, however, if many of these small paths are taken then the cost adds up.
Explanation systems need to give users a sense of the collective cost they will pay of going down all these paths.




\boldify{Unlike other domains/studies where high cost was in navigations (going through stack trace in IDE, debugger, etc), the high cost for our participants was remembering all of the different paths and processing the information they were presented with. }

In \cite{piorkowski2016foraging}, Piorkowski et al. investigated developers ability to predict cost and value.
They found that developers do a poor job of estimating the value they will gain from making navigations, and the cost they will pay to make those navigations.
We noticed that in our study, going down a path would occasionally incur a high cost, such as when Pair 3 had to make seven navigations to find the information they were after.
More significant, however, was the high cost to remember all of the different paths to obtain information and process what information they had obtained. 
Participants had trouble deciding which information to seek at given points, and seemed overwhelmed with game state information.

%One possible reason for this low co-occurrence may be related to  APM, or actions per minute~\cite{wong_2016}.
%Professional players can easily achieve APM values of 300, and APM values can go up to 600 APM during intense battles~\cite{wong_2016}.
%Given that the players in the games we analyzed would all have a high APM, differentiating speed of two player's fighting actions loses meaning because all players could perform these actions at a high speed. 

\boldify{Qualitative coding was performed to analyze how expected and actual value aligned when participants made navigations. }

To analyze how expected and actual value align when participants foraged for information, we looked at responses to the retrospective interview question ``\emph{Did you find what you expected to find?}''
Qualitative coding was performed to categorize the responses into \{yes, no, neutral, or invalid response\}.
We considered responses such as ``\emph{buildings...}'' or when the participant described something such as game content rather than giving a yes or no answer to be ``invalid.''
Meanwhile, responses such as ``\emph{wasn't sure}'' were considered ``neutral.''
Researchers achieved an inter-rater reliability of 97\% on 22\% of the corpus, as measured by the Jaccard index.
After this high level of reliability was achieved, one researcher coded the the rest of the corpus. 

\boldify{Why do we care about ``What else did you consider clicking on''? Here's what it tells us.}

Asking participants to reveal what else they considered clicking on revealed what they missed out on during the course of their navigations.
They often responded with the information they wish they had acquired that they missed out on during the course of their decision making.
The participants had to sacrifice knowledge to acquire what they received.
\FIXME{JED: we discussed how the rewinding runs against this, and I dont think it does.  Going over the video multiple times via rewind has a very high cost (i.e. group 10 spending 1hr analyzing 16m of game)}
%, but the revealing part to information acquisition is the anomalous behaviour that occurred, contrary to previous literature~\cite{piorkowski2016foraging}
%\FIXME{Might need to double check that I'm citing the correct things. MMB: yes, it's wrong.  So I cut the cite.}

\boldify{``I wish I didn't have to make choices ''}

P10 - ``Hmmm if I had multiple, different screens yeah. But no, that seemed to be where the action was gonna be.''\\\\
Humans do not enjoy having to make choices, especially ones that they might come to regret later on.
Participant 10 (P10) commenting on their desire for multiple, different screens to capture as much information as possible reveals that they do not wish to miss things that might be going on in the map.
This means that if participants do not have to deviate from a patch that they are currently deriving information from, they do not. 
\FIXME{JED: Might be worth getting into their manic rewind habit here, seems related}

\boldify{``But seeing as I have to, here's where I missed movement and why it's anomalous''}

Surprisingly, some participants behaved in ways contrary to established human foraging behaviour.
The human visual system is hardwired to see movement.
%they desire to `hunt down' information from visual cues, such as the rustling of a bush or seeing a door creak open.
This translates over to this domain, where participants found their rustled bush in the form of the mini-map.
However, this does not always mean that they followed the anomalous movement.
Participants identified that though there was movement (such as a lot of movement from the AI's base or movement on the mini-map in general), they chose not to attend to this new movement in favour of something else that was currently going on in their field of vision.

\boldify{``However, not all movements are created equally. Some movements are much more pertinent to me than others''}

``I think I considered staying with the mutas, but I saw that there was something else was happening so I decided to check that instead''\\
-  P11 upon seeing a zergling swarm from the south

Movement might naturally catch a human being's eye, but that does not mean to say that all movements are treated equally.
Consider the rustling bush versus a rampaging pack of bulls coming towards you.
Even in instances where the participant was being enriched with information and navigated away from a patch, they considered returning to the source once they had attended to the new event.

\boldify{``In fact, I'm so busy looking elsewhere that I missed the AI moving towards the human player. Here's why this is anomalous''}



\boldify{``Well I might have to make choices, but I'm so fixated on the action that I don't care about the consequence (aftermath)''}

P15 - ``Maybe looking at how that attack, like the aftermath of the attack in that third base.''\\\\

Actions lead to consequence, but participants generally did not seem to care about the consequences of actions that were going on. 
When identifying what they considered looking at, only P15 identified that they would have liked to look at the aftermath of an attack in a base.



\boldify{Expected and actual value aligned 73.5\%  of the time, and misaligned 19.2\% of the time. (The rest were coded as neutral or invalid (when participants did not directly answer the question)).}
\FIXME{MMB to Andrew: We might be able to add a "the road not taken" theme.  To get there, gather up all the times in the utterances where they're saying they had to make a choice (or wish they'd though about the other choices); these are the lost opportunities.  My eyeball scan suggests that you'll find about 50\% they have to sacrifice one choice (foraging paths) to take another.  See if you can somehow group them into different types of phenomena, eg different viewpoints/camera, competing army, other resources of my own, ...}
\FIXME{MMB to Andrew: I'm not buying that there's any real difference in the numbers of "Aligned" vs "Misaligned" below.  Combine into 1 boldification that says what they were looking at (and say that Aligned vs Misaligned were pretty similar) and move on -- maybe to the Whys (very short if they're boring) or maybe to  to "the road not taken".}

%\boldify{Across the data, participants favoured viewing \ValueWhat{combat units} and \ValueWhat{unspecified units}. This indicates that they're far more interested in movement on the mini-map. They also seemed to favour \ValueWhat{building objects}, the collection of which make \ValueWhat{bases}}

%\boldify{The reason that they looked at these objects were generally to \ValueWhy{monitor a game state}, \ValueWhy{attend to new events}, or \ValueWhy{attend to a new event}.}

%\boldify{However, for all that they gained, participants had to prioritise the information that was most valuable to them, sacrificing other pieces of information that could have been important. The data shows that participants preferred to keep their eyes on immediate action with \ValueWhat{combat units}, \ValueWhy{monitoring} them and favouring that information over aftermath events such as \ValueWhat{base} preparation or \ValueWhat{building} actions}

%\boldify{(speaking to interface design) The participants would prefer something with a low navigation cost, seeing as they liked to go to places where there was a high volume of micro activity. Most times that action was going on or that they caught a scent that armies were on the move, participants preferred to go to them, abandoning current tasks such as scouting around bases}


%\boldify{Across all yes and no responses to value alignment, participants were looking at \ValueWhat{Combat Units} (39.26\%), the \ValueWhat{bases} (17.04\%), and \ValueWhat{building objects} (14.07\%), and their top reasons for looking were \ValueWhy{monitoring-game-state} (44.44\%), \ValueWhy{attend-new-event} (22.22\%), and \ValueWhy{Updating-Stale-Game-Info} (20\%)}

%\boldify{When expected and actual value did align, participants were looking at \ValueWhat{combat units} (40.19\%), the \ValueWhat{bases} (19.63\%), and \ValueWhat{unspecified units} (14.02\%).}

%\boldify{When expected and actual value did not align, participants were looking at \ValueWhat{combat units} (35.71\%), \ValueWhat{buildings} (28.57\%), and \ValueWhat{unspecified units} (10.72\%) }

%\boldify{We now know what the participants are looking at, so why do they look at these? Well, our data revealed that when value aligned, the priorities placed on why was \ValueWhy{monitoring a game state} (42.99\%), \ValueWhy{attending to a new event} (24.3\%), \ValueWhy{updating stale game information} (18.69\%), and \ValueWhy{updating stale domain information} (5.61\%) }

%\boldify{When values misaligned, the priorities that participants identified to justify their navigations were \ValueWhy{monitoring a game state} (50\%), \ValueWhy{updating stale game information} (25\%), \ValueWhy{attending to a new event} (14.29\%), and \ValueWhy{updating stale domain information} (10.71\%)}

\FIXME{This stuff above was what was in ResultsValue.tex}

\boldify{We found that the majority (140/202) of questions, and in particular a majority (103/148) of \LimDey{What} questions, came from two pairs in particular (3 and 10). Furthermore, participants within these pairs asked \LimDey{What} questions an equal amount.
We noticed two things participants in these pairs had in common: They were more likely than our average participant to have experience with the original StarCraft, but less likely to be in a current StarCraft 2 ladder. Perhaps participants who have experience with an older version of the system, but not in depth knowledge of modern system, may ask more questions when debugging an intelligent agent. }

We noticed that participants who asked the most questions had similar backgrounds, suggesting that test pilots with this type of background may use an explanation system in this way.
Pairs 3 and 10 asked most of the questions (140/202), and most (103/148) of the \LimDey{What} questions, 
In pair 3, P5 asked 19 \LimDey{What} questions while P6 asked 22 \LimDey{What} questions, and in pair 10 both participants asked 31 \LimDey{What} questions.
To explain these numbers, we look to participant demographic information and experience. 
None of these four participants were in a league on the StarCraft ladder, while 50\% of our participant population were in a league.
Across all 20 participants, only 30\% listed experience with the original StarCraft (StarCraft 1 and StarCraft: Brood War).
Of the participants in pairs 3 and 10 a much higher amount, 75\%, listed experience with the original StarCraft.
Perhaps when test pilots have knowledge of a previous iteration of a system an intelligent agent is working in, but less in depth knowledge of the newer system, test pilots will ask more questions when debugging the agent.

Other events led participants to asking \LimDey{Why} questions, such as confirming why they thought an action was performed. 
For example, P19 asked ``And in response he started building another Hatchery, right?''

\boldify{Most of the \LimDey{Why-did} and \LimDey{Why-didn't} questions came from session 10. Surprisingly, it was the participant with more experience that was asking these questions.}

The majority of \LimDey{Why-did} and \LimDey{Why-didn't} questions came from Pair 10 (P19 and P20).
At first, one might expect the less experienced participant to ask the \LimDey{Why-did} and \LimDey{Why-didn't} questions, because someone with less experience may not know why actions were performed as part of a player's strategy.
In this case, it was the player with more experience, P20, who asked more \LimDey{Why-did} and \LimDey{Why-didn't} questions.
P20 asked 5 \LimDey{Why-did} and 4 \LimDey{Why-didn't} questions, while P19 asked 3 \LimDey{Why-did} and 1 \LimDey{Why-didn't} questions.
P20 had 145 hours of experience across all RTS games they played, while P19 only had 10 hours of experience across all RTS games.
According to Lim \& Dey \cite{lim2009assessing}, users demand less \LimDey{Why} explanations when expectations are not violated.
The more experienced player, P20, must have had expectations violated by the agent, therefore asking more \LimDey{Why} and \LimDey{Why-didn't} questions.
Indeed, P20 asked questions when the agent performed actions they did not expect, such as when P20 wondered ``What was the point of that?'' when investigating scouting actions. 

\boldify{Interestingly, we found that those with expertise in other areas of RTS asked different questions}

\FIXME{**FAKE RESULT 2: The domain experts that we investigated all had similar backgrounds, with a minimum of 10 hours in StarCraft, but we also noticed that participants brought in knowledge from other games, such as Command \& Conquer, Age of Empires, or Rome: Total War.
We wished to investigate if ``Jake'' might ask different kinds of intelligibility type questions if he brought a background that had a similar domain, in this case RTS games, but with a variant type than what he sees before him.
What we noticed was that those participants that had extreme comfort with the game itself, measured by those with x number of hours, asked a lot of \LimDey{Why} questions, attempting to delve deeper into the background behind an event that they had witnessed.
However, those that did not have as much familiarity, or at least those that had logged more hours into other RTS games, asked a lot more about \LimDey{What}, catering their foraging behaviours towards gaining more knowledge that was specific to the game.
tl;dr: I want to know if ``Jake'' will care about different kinds of information. In a real world example, suppose we have an expert pilot that is used to flying commercial airlines, but we then take him over to a military flying operation.
This is a similar domain (flying) but different knowledge needed (faster planes, turning circles, etc)
}

One of these participants, P6, was much more likely to navigate for the purpose of updating stale domain info.
From answering RQ1, we saw that participants navigated in order to update stale domain info 11 times, and 5 of these were from P6.

 
\boldify{Implications ideas: 1. sufficiency of descriptive language - explanation systems could be modeled after shoutcasters if there is match between users and caster, 2. why language being tied to expectations, both at the level of expectations met or not met (build was standard, consult group 4+5) and at the level of expectation of getting an ANSWER.  I.e. asking why he didnt move zerglings doesnt do a lot when no one in the room knows.  maybe they didnt ask.  Meanwhile, lim-dey provide a mechanism by which asker had reasonable expectation to obtain answer.}

% Looking for patch types that users wished were there, not the patch types that were actually there. We'll be attending to the cues.
% Whats help us to define not only the prey but also what types of patches should have been there.
% It seems like part of the whys has to be a cue. Known v UnKnown. Cues they found value in and cues that they wished were there. Map activity is a dynamic cue, and some kind of cue 
% Stale information is lost scent. Hungry and foraging around for a rabbit. 
% monitoring reasonable thing to have with cue or being responsible or could subcode by the three subtypes


The most popular type of Lim \& Dey question users asked aligned reasonably well with the most popular answer shoutcasters provided, suggesting that an explanation system in this domain could be designed based on shoutcaster explanations in that regard. 
We need to be careful when building these explanation systems, however,  because within categories of Lim \& Dey questions such as \LimDey{What}, specific types of questions/answers can widely vary. 
Some of the \LimDey{What} questions are very broad, asking in general what is going on.
It may be more difficult for explanation systems to respond to these types of questions where the user is not asking for specific information. 

------------------------------------
\FIXME{What follows is the old RQ-paths version}

\boldify{Metaphor is a processor (could be trails in the woods, but would require teleportation to really be clear).
The processor starts with nothing to do. Then a marine is made! Its actions receive a great deal of scrutiny because it is the only thread on the processor}

During the preliminary stages of a StarCraft II match, there is very little going on in the environment.
This is similar to how just after a computer boots, there are very few threads on the processor to choose from.
As such, keeping track of these threads is a reasonably easy task.
When this is the case, the performance is easily evaluated, and each thread finds itself under a great deal of scrutiny.
Within the first minute of the game, or a few seconds after, four different pairs paused the replay for an average of 57 seconds.
Drawing back to StarCraft II, the early stages come under a great deal more judgment, but everything that exists on the map is easy to keep track of.
\Pair{P14} encapsulated this idea perfectly during the early game: \quotateUnattrib{There is only so many places to click on at this point.}

\boldify{The player expands! this creates another thread.  This repeats a bunch of times. Now the processor has a bunch of threads to service (skipping back and forth between threads).}

As the complexity of the StarCraft II game develops, so too does the complexity of the participants' task; there's an inherent need to keep track of many different ideas (threads) at one time.
This translates neatly over to the CPU analogy, which is now running many threads.
The participants had to keep track of a great deal of information that is being displayed currently in the match.
Our data reflected this when, during the post-task interview, we had asked participants ``\emph{What made you click on this aspect of the interface.}''
From Table \ref{table:whyCoding}, we saw that 
\ValueWhy{Stale Game} was the reason for 20\% of participant navigations.
When making these navigations, participants were updating their knowledge of game information that they explicitly stated prior knowledge about (executing a thread that was previously generated and suspended).


%\boldify{Some threads are killed; e.g. the tester sees a pile of zerglings has clearly been forgotten about and concludes ``bad agent action''}

\boldify{But more threads are forgotten because many increasingly important threads are created. e.g. the actions of that first marine no longer get the same scrutiny late in the game, theres just too much other stuff! This maps to ``New Event'' in the ``Why'' coding.}

Similarly, humans can only keep track of a certain amount of ideas at one time.
As time passes in the RTS environment, threads continue to appear, meaning each process will not receive the same degree of scrutiny that it may have when it was among many fewer process being executed.
As such, people tend to forget about the actions of certain units, corresponding to a thread being ignored by the scheduler, as more pressing, newer threads are created and executed.
\Pair{P19} commented during the main task about the complexity of their task, stating: \quotateUnattrib{There's just so much happening all at once; I can't keep track of all of it!}
From Table \ref{table:whyCoding}, we saw that attending to a \ValueWhy{New Event} was the reason for 26\% of navigations. 
\ValueWhy{New Event} referred to any new event that participants were curious about and explored, for example:
\quotateInset{10}{19}{...noticed movement in the Minimap, and that the Zerg troops were mobilizing in some fashion.  So I guess I just preemptively clicked...}
%Furthermore, they accentuated this point in the post task, highlighting the importance of making the multiple areas of information readily available: P19: 

\FIXME{JED @ MMB: this paragraph is the main one that I think comes through strongly as a CPU analogy, but falls pretty flat as a forest trail analogy.  The other ones I can envision better how we might reframe as trails.}

\boldify{In the presence of things being forgotten, people acted several different ways. 
1. Rewind/pause/slow down and 2. soldier on and ignore it:}
% Claudia loop behaviour quote: ''okay, so I looped back to the beginning of the final fight cause I wanted to see if there was anything significant that we had missed the first time around""

Since participants found the task exceeded their ability to track everything, they responded in several ways, with the first being to slow down the replay or rewind parts of it.
As Table~\ref{table:taskTime} indicates, 7 \Pair{Pairs} rewound the replay at least once, while 3 \Pair{Pairs} decreased the speed of the replay.
Every participant group paused the replay, though many of these were to fill out forms as opposed to examine the gamestate more thoroughly, (which would be more similar to using a breakpoint and a debugger to more thoroughly examine program execution state)
However, note from Table~\ref{table:taskTime} that the \Pair{Pairs} which chose to extensively rewind the replay (\Pair{Pairs 3} and \Pair{10}) spent substantially more time than their counterparts.
Most \Pair{Pairs} took between 20 and 40 minutes, while the two who heavily rewound took around an hour.
\FIXME{JED: thats not entirely true, my read of it was that one took an hour due to rewind, the other took that long due to watchig the WHOLE replay at a slow speed + some rewinds.}
Note that the replay was 16:04 long, so a shoutcaster would be forced to finish their analysis within that 16 minute window.
Many \Pair{Pairs} analyzed the replay using not much more time than the shoutcasters would have spent.
Achieving this speed of analysis required \Pair{Pairs} to \emph{ignore} many game events.

\boldify{ Participants generally ignored a human instinct for attending to movement in order to gain information from another, better movement. However, not all movements are created equally; participants had to prioritize where they were looking at to stay ``with the action''}

Humans have a natural instinct towards attending to movements, such as the rustling of a bush that they see out of the corner of their eye.
This translates over to the RTS domain, when they see sudden movements in the mini-map that they believe might lead to more valuable information than what they are receiving currently.
However, not all movements are created equally.
As the number of threads increase, prioritization must occur, since the human can only keep track of a finite field of vision at any one time.
\Pair{P19}, during the post-task interview when asked if they desired to click elsewhere, stated: \quotateUnattrib{Mmm, if I had multiple, like, different screens yeah. But no, that seemed to be where the action was gonna be.}
This demonstrates that choices \emph{must} be made, and even though \Pair{P19} wished to derive information from elsewhere on the map, they lacked the means by which they might achieve this desired behavior.

\boldify{Replenishing (production) > current fight\\ The prioritisations that the participants identified lead to a partial ordering, and it became evident that replenishing lost forces was of more importance to the participants than a fight currently going on.}

\Pair{Pairs} prioritized attending to replenishment of forces that had recently been lost, over attending to the last part of a fight.
For example:
\quotateInset {6}{11}{I think I wanted to check on his production that one time, because he just lost most of his army, and he still had some protoss to deal with.}
This ordering makes sense, since \Pair{Pairs} would want to know how the opposition was going to prepare for lost resources or for the possibility of a counter-attack.
\FIXME{JED: I dont understand the ``preparing for lost resources'' part}
Furthermore, Participant 5 stated, while a fight was wrapping up elsewhere on the map: \quotateUnattrib{I was trying to see what units they were building, after the fight, see if they were replenishing, or getting ready for another fight.}
\Pair{Pairs} wanted to see how the agent that they were keeping track of was preparing for a move or two ahead, as opposed to wanting to stay with the action.
This is logically sound, since any one fight could help sway the battle in any favour, so participants wanted to know how preparation is going for the next combat that will inevitably commence.
\FIXME{JED: we arent proving anything, so soundness doesnt help us, rephrase somehow.}


%Claudia replenishing units quote:``I think I wanted to check on his production that one time, because he just lost most of his army and he still had some protoss to deal with''

\FIXME{SP: I think we may want to replace this whole ``hierarchy'' discussion since we don't have any numbers to prove it.  We make want just make the next couple paragraphs about `Here's what some participants chose to prioritize instead of going down certain paths''}

\boldify{Large Force > harassment\\Participants also identified that they care about the size of clusters more, and a bigger ``bush'' will attract their attention more than a smaller one. This was demonstrated when a large force approaching from another location was more important to them than an ongoing harassment.}

\Pair{Pairs} attending to motion identified that the size of movement was a factor taken into consideration, such as \Pair{P11}'s identifying the following:
For example, a large force coming to attack was of more importance than an ongoing harassment. 
\FIXME{JED: I think this quote got butchered somehow in the formatting. Not really sure what happened here}
\Pair{P11} stated that during a harassment by some mutalisks (mutas): \quotateUnattrib{I think I considered staying with the mutas, but I saw that there was something else was happening so I decided to check that instead.}
\FIXME{JED: telling them that mutas are mutalisks will help approximately no one.  maybe tell them they are a fast, flying attacker?}
The something else that the participant identified was a large force of the Zerg coming from the south to attack the Protoss. 
\FIXME{JED: We have not defined zerg or protoss, avoid using them}
This reply was in response to being asked if they considered clicking anywhere else, and it is clear to see that information had to be given up (the harassing actions of the mutalisks) to attend to a potentially greater `threat' in the form of the attack coming from the south.

\boldify{current fight > expected fight\\Though there could be the scent of an anticipated fight from movement in the mini-map or based upon the clustering and arrangement of forces, participants preferred to stay with the ongoing action as opposed to attending to the anticipated collision}

As stated above, participants enjoyed staying with the action, wishing to try to gauge a success or failure of the battles at hand.
Anticipated fights are ones that can be inferred, similarly to how a wolf hunts a deer, from the ``scent'' coming from the mini-map.
This should metaphorically turn heads, but what our participants generally did was try to stay with the action rather than attend to action that would potentially happen.
This was shown when participants revealed their intention in the main task or reflected upon their actions in the post-task, desiring to stay with a current action than to see expansions elsewhere or other units engaging in combat.

\FIXME{JED: I had a hard time following this paragraph's point. possible cut since it does not present any data?}


\boldify{This hierarchy sometimes lead participants to take such focus in certain areas, attending to rustling bushes, that they could not attend to what might be deemed as more pressing information, such as an enemy attack coming.}

Since a hierarchy of desired information can be inferred, the complexity of the game as time goes on proves a challenge for participants to continue making these choices.
\FIXME{JED: I do not think that we have established that a hierarchy CAN in fact be inferred (we are merely hypothesizing it can, and the section up to this point does not prove this hypo}
After all, when there are dozens of rustling bushes, a predator might not know which bush to investigate that will reveal the most valuable prey.
Since this is the case, when the predators makes the choice, it is possible that the prey that exists in one of these other bushes might have been more pertinent to them or more pressing.
The participants revealed this for us, especially in instances where they either did not notice or did not feel it necessary to attend to an action that could have costly consequence, such as an enemy attack or a behavior that was detrimental economically, such as the elimination of workers.
[Would like a participant quote here]
This quote was in response to the question ``did you consider clicking anywhere else,'' and it shows that this hierarchy of desired viewing does come with a cost, and some threads never really get closed or formally investigated.

\FIXME{JED: after reading this far, I am still not buying that we have demonstrated a hierarchy\\
AAA: Yeah even as the author of this section, I'm not entirely convinced that what I thought was there was actually there. However, cutting out the last 3 paragraphs will lead us to a very small section.\\
I'm more than open to suggestions that you might have as to how best to rephrase or to rework this section such that it fits better in with Decision Points.}


\boldify{Implications: we need to encourage threads being closed formally and not being forgotten. i.e. if a tester asks WHY an agent did a thing, it may be worthwhile asking the tester to JUDGE that action at some point after they are able to look into it. Keeping between 5-10 threads somehow}

Taking into consideration the hierarchy discussed and how the participants had to sacrifice potential information for feeling that they could be enriched by another location, our data supports that we need to enable the user ``Jake'' to close threads of investigation and not forget about important lines of inquiry.
For example, if a tester asks the agent WHY it performed an action, the tester should be able to judge the quality of an agent's actions.
In an effort to promote the closure of threads, a couple of different paradigms could be adopted.
On one hand, the interface could interact with ``Jake'' in real-time to promote awareness of threads that might have become stale or are on the verge of being forgotten.
Due to the complexity of the StarCraft II domain, it might be worthwhile investigating ways to minimize the amount of threads that an agent must keep track of at any one time.
Should a thread be forgotten, similarly to how Participant 19 felt, the system should be able to react accordingly to explain why it is making certain actions or bring to the attention of the user information that becomes necessary at the right time.
A to-do list may reduce the cognitive load, which was utilized by a debugging tool for spreadsheet programming in \cite{grigoreanu2010strategy}.
This allowed users to keep track of what to return to later, and monitor what they have looked at vs what they skipped.
A to-do list may also be useful in the domain of RTS games, given the problems our participants had.

\FIXME{JED: this paragraph is too long. I would crack it in half, where first we identify and quantify the problem (threads being forgotten, because of too many threads which are potentially long). and another paragraph where we recommend fixes (judgment, TODO list, etc)}

%%%%%%%%%%%%%%%%%
% \input{tables/TableParticipantExperience}
% MMB: goes in methodology. And not this format -- we want an individual list
%%%%%%%%%%%%%%%%%

\FIXME{End of the old RQ-paths version}
------------------------------------

\FIXME{This is the old Analysis section-----------}

\boldify{Elements of the corpus that were used for analysis included the main task interview, post task interview, and decision point forms.}

To answer RQ1, we qualitatively coded instances in the main task where participants asked a question out loud.
To answer RQ2, we qualitatively coded from the retrospective interview answers from participants about interface navigation questions. 
To answer RQ3, we qualitatively coded data from the decision point forms the participants completed.

\boldify{We examined key decision points users identified. Groups of decisions points were identified during an affinity diagramming session, and qualitative coding was then performed using the groups to guide the coding.}

Key decision points users identified were classified into groups during an affinity diagramming session.
The four higher level groups we identified were building/producing, scouting, moving, and fighting.
We coded 56 of the 228 identified decision points, and reached IRR of 80\%, at which point one researcher coded the rest of the data, shown in more detail in Table~\ref{table:decisionPointsSummary}.

\boldify{Lim Dey coding was performed to answer RQ4.  Our researchers had previously achieved IRR on another corpus, which we argue carries over to this corpus.}

Utterances where participants asked a question during the main task were coded using the code set outlined in Table \ref{table:limDeyCoding}.
Our researchers have used the same coding schema on a different corpus [Removed for anonymized review] in which they independently coded 34\% of the corpus and achieved 80\% inter-rater reliability.  
The researchers who achieved sufficient IRR during the previous study coded the corpus for this study.

\boldify{Affinity diagramming and qualitative coding was performed to answer the question ``Why was the participant seeking information.''}

In order to answers the question ``\emph{Why was the participant seeking information?}'' we initially performed affinity diagramming to generate groups of answers.
From the affinity diagram, the codes we generated were \ValueWhy{Monitoring State}, \ValueWhy{Updating Game State}, \ValueWhy{Obsolete Domain}, and \ValueWhy{New event}, as shown in Table~\ref{table:whyCoding}.
Qualitative coding was then performed on the groups we generated from the affinity diagramming.
Using that code set, we achieved IRR of 80\% on 20\% of the corpus, at which point one researcher completed the rest of the coding.

\FIXME{----------end of the old Analysis section}





==> z-DraftCommands.tex <==
\newcounter{boldifyCounter}
\newcounter{fixmeSectionCounter}
\newcounter{fixmeTotalCounter}

%%%%%%%%%%%%% Drafting commands %%%%%%%%%%%%%%%%%%%%%%

\newcommand{\boldify}[1]{%
\stepcounter{boldifyCounter}%
\textbf{{\color{green}**}%
~\arabic{section}.\arabic{subsection}.\arabic{boldifyCounter}%
: #1}}

\newcommand{\FIXME}[1]{%
\stepcounter{fixmeSectionCounter}\stepcounter{fixmeTotalCounter}%
\fbox{%
\parbox{\linewidth}{%
\textbf{FIXME \arabic{section}.\arabic{subsection}.\arabic{fixmeSectionCounter} (\color{red}\#\arabic{fixmeTotalCounter}):} #1}}
}


\addtocounter{fixmeSectionCounter}{-2}
\addtocounter{fixmeTotalCounter}{-2}
\makeatletter
\@addtoreset{fixmeSectionCounter}{section}
\@addtoreset{fixmeSectionCounter}{subsection}
\@addtoreset{boldifyCounter}{section}
\@addtoreset{boldifyCounter}{subsection}
\makeatother


%%%%%%%% DRAFT HEADER//FOOTER STYLING COMMANDS %%%%%%%%
\usepackage{fancyhdr}
\pagestyle{fancy}
 
\fancyfoot{}
\renewcommand{\footrulewidth}{1pt}
\pagenumbering{arabic}
\lfoot{Page~\thepage}
\cfoot{\currenttime~GMT~(PST is GMT-07:00)}
\rfoot{\today}
